SGP-TOD: Building Task Bots Effortlessly via Schema-Guided LLM Prompting

Building end-to-end task bots and maintaining their integration with new functionalities using minimal human efforts is a long-standing challenge in dialog research. Recently large language models (LLMs) have demonstrated exceptional proficiency in conversational engagement and adherence to instructions across various downstream tasks. In this work, we introduce SGP-TOD, Schema-Guided Prompting for building Task-Oriented Dialog systems effortlessly based on LLMs. Utilizing the symbolic knowledge -- task schema, we instruct fixed LLMs to generate appropriate responses on novel tasks, circumventing the need for training data. Specifically, SGP-TOD comprises three components: a LLM for engaging with users, a DST Prompter to aid the LLM with dialog state tracking, which is then used to retrieve database items, and a Policy Prompter to elicit proper responses adhering to the provided dialog policy. Experimental results on Multiwoz, RADDLE and STAR datasets show that our training-free strategy SGP-TOD, without any task-specific data, yields state-of-the-art (SOTA) zero-shot performance, greatly surpasses the few-shot approaches. In a domain-extension setting, SGP-TOD aptly adapts to new functionalities by merely adding supplementary schema rules. We make our code and data publicly available.

==> section/backup.tex <==
% \begin{table*}[!t]
%     \fontsize{6}{6}
%     \selectfont
%   \centering
%   \begin{threeparttable}
%     \begin{tabular}{lcccccccccccccccc}
%     \toprule  
%     \multirow{2}{*}{Model} &
%     \multicolumn{4}{c}{\texttt{Attraction}}&\multicolumn{4}{c}{\texttt{Train}}&\multicolumn{4}{c}{\texttt{Hotel}}&\multicolumn{4}{c}{\texttt{Restaurant}}\cr  
%       \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
%       &$\mathtt{Info.} $&$\mathtt{Succ.}$&$\mathtt{BLEU}$&$\mathtt{Comb.}$&$\mathtt{Info.}$&$\mathtt{Succ.}$&$\mathtt{BLEU}$&$\mathtt{Comb.}$&$\mathtt{Info.}$&$\mathtt{Succ.}$&$\mathtt{BLEU}$&$\mathtt{Comb.}$&$\mathtt{Info.}$&$\mathtt{Succ.}$ &$\mathtt{BLEU}$&$\mathtt{Comb.}$ \cr 
%     \midrule
%     \multicolumn{17}{c}{Zero-shot prompting}\cr  
%      \cmidrule(lr){1-17}
%      SP-TOD-Codex  & 98.00 & 93.00 & 10.45 &105.95 &78.79 & 70.20 & 8.56 & 83.06 &83.50 & 69.50 & 7.86 & 84.36 & 91.00&85.00&10.50 &98.50\\
%     \midrule
%     -policy & 98.00 & 90.00 & 9.08 &103.08 &60.10 & 57.07 & 5.82 & 64.41 &72.00 & 40.00 & 5.62 & 61.62 & 71.00&61.50&9.68 &75.93\\
%     -policy-CoT & 95.00 & 92.00 & 8.82 &102.32 &74.24 & 61.62 & 7.86 & 75.79 &70.00 & 22.00 & 6.18 & 52.18 & 73.50&58.50&10.00 &76.00\\
%     -policy-CoT-Belief & 84.00 & 77.00 & 8.92 &89.42 &77.78 & 67.17 & 8.15 & 80.62 &61.50 & 26.50 & 5.90 & 49.90 & 45.00&34.00&9.64 &49.14\\
%     \bottomrule  
%     \end{tabular}
%   \end{threeparttable}
%   \caption{End-to-end evaluation on \texttt{Multiwoz}.
%   }
%   \label{tab:results_4task}
% \end{table*}


% \begin{table*}[!t]
%   \centering
%   \begin{threeparttable}
%   \fontsize{7}{7}
%   \selectfont
%     \begin{tabular}{lccccc}
%     \toprule
%     % \multirow{2}{*}{Model}&\multirow{2}{*}{\texttt{Task}}&\multirow{2}{*}{\texttt{Schema types}}&\multicolumn{2}{c}{\texttt{Training strategy}}\cr\cmidrule(lr){4-5}
%     % &\texttt{Fine-tuning/Pre-training}&\texttt{In-context learning} \cr
%     % \midrule
    
%     % \multicolumn{5}{c}{\Checkmark with 2.5k training dialogs}\cr  
%     %  \cmidrule(lr){1-5}
%     \multirow{2}{*}{Model}&\multirow{2}{*}{\texttt{Task}}&\multirow{2}{*}{\texttt{Schema types}}&
%     \multicolumn{3}{c}{\texttt{Training strategy}}\cr\cmidrule(lr){4-6}
%          &&&\texttt{Fine-tuning}&\texttt{Pre-training}&\texttt{ICL} \cr
%     % \midrule
%     \midrule
%     RobustSF\cite{shah2019robust} &SF&\cellcolor{cyan}slot names/value examples&\Checkmark \\
%     % \midrule
%     \midrule
%     TRADE\cite{wu-etal-2019-transferable} &DST&\cellcolor{cyan}slot names/value examples&\Checkmark\\
%     ZSTL-SD\cite{campagna-etal-2020-zero}&DST&\cellcolor{orange}{ontology, representative dialogs}&\Checkmark(+synthesized-data) \\
%     % S-DST\cite{rastogi2020towards}&DST& service, intent, slot names/descriptions&\Checkmark\\
%     \cmidrule(lr){3-3}
%     \multirow{2}{*}{S-DST\cite{rastogi2020towards}}&\multirow{2}{*}{DST} &\cellcolor{pink!70}{slot names/descriptions} &\multirow{2}{*}{\Checkmark} \cr &&\cellcolor{magenta}{+service, intent names/descriptions} \\
%     \cmidrule(lr){3-3}
%     T5DST\cite{lin2021leveraging} &DST&\cellcolor{pink!70}{slot names/descriptions}&\Checkmark\\
%     TransferQA\cite{lin2021zero} &DST&\cellcolor{cyan}slot names/value examples&&\Checkmark(QA tasks)\\
%     IC-DST\cite{hu-etal-2022-context} &DST&\cellcolor{cyan}slot names/value examples&&&\Checkmark\\
%     % Multi-Bert\cite{kapelonis22_interspeech} &DST&&In-context learning\\
%     SDM-DST\cite{wang-etal-2022-slot} &DST&\cellcolor{cyan}slot names/value examples&\Checkmark\\
%     \midrule
%     Bert+S\cite{mosig2020star}&E2E policy&\cellcolor{brown}{system-side policy skeletons}&\Checkmark\\
%     SAM\cite{mehri2021schema} &E2E policy&\cellcolor{brown}{user-aware policy skeletons}&\Checkmark\\
%     \midrule
%     ZSDG\cite{zhao2018zero} &E2E dialog&\cellcolor{orange}{ontology, representative dialogs}&\Checkmark \\
%     DAML\cite{qian-yu-2019-domain} &E2E dialog&\cellcolor{orange}{ontology, representative dialogs}&\Checkmark \\
%     % AnyTOD\cite{zhao2022anytod} &E2E dialog&slot, action names/states/descriptions, policy programs&\Checkmark&\Checkmark(heterogeneous tasks)\\
%     \midrule
%     \multirow{4}{*}{AnyTOD\cite{zhao2022anytod}}&\multirow{4}{*}{E2E dialog}&\cellcolor{brown}{policy program} &\multirow{4}{*}{\Checkmark}&\multirow{4}{*}{\Checkmark(heterogeneous tasks)} \cr &&\cellcolor{blue}{+slot names/value examples} \cr
%     &&\cellcolor{pink!70}{+slot descriptions} \cr &&\cellcolor{purple}{+action names/states/descriptions} \\
%     \cmidrule(lr){3-3}
%     \multirow{2}{*}{IC-TOD(ours)}&\multirow{2}{*}{E2E dialog}&\cellcolor{brown}{user-aware policy skeletons} &&&\multirow{2}{*}{\Checkmark} \cr &&\cellcolor{blue}{(+slot names/value examples)} \\
%     \bottomrule  
%     \end{tabular}
%   \end{threeparttable}
  
%   \caption{Zero-shot task-oriented dialog modeling. (The schema items in the parentheses are needed only when they are available.)}
%   \label{tab:related}
%   \vspace{-1mm}
% \end{table*}


    %AnyTOD-XXL \cite{zhao2022anytod} is a schema-guided approach implemented on T5-XXL \cite{roberts2022scaling}, which is pre-trained on SGD \cite{DBLP:conf/aaai/RastogiZSGK20}\footnote{SGD is a large-scale schema-guided multi-domain dialog dataset, spanning 45 domains.}. AnyTOD-XXL first tracks dialog states and action states using a description-driven neural model.

    %, which limits the widespread adoption of such systems.
    \cellcolor{pink!70}{\makecell[l]{\textbf{System:} I'm sorry, but \textcolor{red}{I could not find any information} \\\textcolor{red}{on delivery fee} in our database. You may want to contact \\ the restaurant directly to inquire about this. Is there \\anything else I can assist you with today?}}

    (\eg ChatGPT\footnote{
\url{https://chat.openai.com/}}, GPT-3 \cite{NEURIPS2020_1457c0d6}, Codex \cite{chen2021evaluating}) 

%In this work, we use 2688 single-task dialogs, which follow a happy path, \ie the user is not instructed to do anything that go beyond what the schema anticipates. 

%%%%%%%%%%%%%%%%%%%%%
% $(\RN{5})$ Restaurant-ext \cite{zhang2022toward} is a single-domain dataset, constructed via extending the original Restaurant dataset in RADDLE \cite{DBLP:conf/acl/PengLZZLG20}, following the domain extension setting \cite{lipton2018bbq}. Specifically, each dialog is expanded to include four additional slots about new functions \ie recommendation for restaurants' trademark dishes (\textit{[restaurant\_dish]}), delivery service (\textit{[value\_price]}, \textit{[start\_time]}, \textit{[end\_time]}). All database entries in the backend database are updated with corresponding values. 10/50/50 examples are provided in Restaurant-ext for training, validating, and testing.


In this work, we propose SP-TOD, a schema-guided prompting method for zero-shot end-to-end task-oriented dialog modeling. Specifically, we incorporate the pre-defined task schema and dialog context into the prompt to instruct LLMs to generate appropriate responses on new tasks. Such training-free design enables developers to effortlessly and quickly prototype dialog systems on new tasks using merely task schema and little annotation. To achieve trustworthy dialog modeling, we formulate the end-to-end dialog generation as a multi-step reasoning problem, where the LLM tracks belief state based on the dialog context, fetches matched entry from database using the belief state, and then elicits appropriate system action and corresponding response (i.e, chain-of-thought prompting \cite{wei2022chain}). By fusing the database expertise with the powerful reasoning, language understanding, and generating capabilities of LLMs, IC-TOD provides knowledge-based, easily interpretable and user-friendly responses.

that not only are grounded in dialog states but also adhere to the pre-defined dialog policy. 

\subsection{Human Evaluation Metrics.}

\subsection{Database retriever}
Database retriever endows the LLM with the capability of grounding their responses on external knowledge for task completion, reducing hallucination. Specifically, as shown in the upper left corner of Figure \ref{fig:operation_process}, the retriever first generates the search query based on the generated belief state, then it calls task API to query the task-specific database for matching DB entry(s), finally it returns the result set of the retrieved entry(s) to the frozen LLM.


%% task definition and significance
Neural-based task-oriented dialog (TOD) systems have achieved impressive performance in facilitating user completion of a wide range of tasks via natural language interaction. 
% main challenge, example
%Dialogue systems face the problem of
One major challenge in developing such systems is to flexibly adapting them to new tasks or domains to satisfy the ever-expanding user/business requirements \citep{mehri2021schema,zhang2022toward}. For instance, to endow a hotel bot with the ability to book taxi typically requires adequate data to be collected and annotated, which is costly and time-consuming. As a result, zero-shot dialog modeling—in which a dialog system picks up new skills without additional training corpora—becomes fairly important yet remains understudied.

% current work, categories, problems to be solved, example
There are two major study axes in zero-shot dialog modeling. The first axis \cite{zhao2018zero,qian-yu-2019-domain} relies on finding a shared dialog policy to transfer the agents from the source domain to the target domain. Yet, in real-world scenarios, the dialog policy may vary dramatically from task to task. In order to enable boarder adaptation to unseen tasks/domains with varied dialog policies, the second one \cite{mosig2020star, zhao2022anytod, mehri2021schema} employs the schema-guided paradigm to explicitly direct the agents to execute on new tasks in a zero-shot manner with the injected task schema, which describes the dialog policy of the new task. However, in order to train the agents to follow the task schema, these approaches need training them on a large number of rich-resource source/heterogeneous domains/tasks with sufficient annotations (\eg state descriptions, action descriptions, \etc). 

Recently, large language models (LLMs), such as GPT-4 \cite{openai2023gpt4}, ChatGPT\footnote{\url{https://chat.openai.com/}} and GPT-3 \cite{NEURIPS2020_1457c0d6}, have demonstrated an astounding ability to produce human-like, coherent, and informative replies on a variety of open-domain tasks. Nevertheless, they have trouble handling specific specialized duties in real-world circumstances, \ie providing false information or being unable to address inquiries regarding particular functionality, due to a lack of database expertise and domain-expert knowledge. To equip LLMs with external knowledge, \citet{DBLP:conf/emnlp/ZhongLC22} proposes fine-tuning an LLM's parameters, which can be quite time-consuming and prohibitively expensive as LLMs get more and bigger.

% to solve the problem, propose model, including parts, each part functionality, performance, (techniques).

In this work, we propose SP-TOD, a schema-guided prompting method for zero-shot end-to-end task-oriented dialog modeling, where we incorporate the pre-defined task schema and dialog context into the prompt to instruct fixed LLMs to generate appropriate responses on any novel tasks in a zero-shot manner (without any pre-training/fine-tuning). Specifically, SP-TOD comprises four components: $(\RN{1})$ a frozen LLM for communicating with users, $(\RN{2})$ a DST prompter for helping the LLM track dialog states based on the dialog context, $(\RN{3})$ a database retriever fetches matched entries from a database using the generated dialog states, $(\RN{4})$ a policy prompter directs the LLM to generate appropriate responses that adhere to the pre-defined dialog policy. By fusing the database expertise, domain-expert knowledge with the powerful language understanding and generating capabilities of LLMs, SP-TOD provides knowledge-based, easily interpretable and human-like responses. Moreover, such training-free design enables developers to effortlessly and quickly prototype dialog systems on new tasks using merely task schema and little annotation. 

We conduct empirical experiments on two multi-domain datasets: Multiwoz 2.0 and 2.2 \cite{budzianowski2018large,zang-etal-2020-multiwoz} and two single-domain datasets: RADDLE \cite{budzianowski2018large,peng2021soloist} and STAR \cite{mosig2020star} in zero-shot settings. Results demonstrate that SP-TOD, \textit{without any pre-training/fine-tuning} $(\RN{1})$ significantly outperforms the current state-of-the-art (SOTA) zero-shot transfer model, which is pre-trained on SGD dataset \cite{DBLP:conf/aaai/RastogiZSGK20} and achieves competitive performance with full-shot fine-tuning methods on Multiwoz 2.0 and 2.2; $(\RN{2})$ achieves superior performance than few-shot fine-tuning methods on RADDLE; $(\RN{3})$ achieves respectable performance on STAR compared to SOTA zero-shot transfer models, which are first fine-tuned on massive amounts of source data. Furthermore, in the domain-extension setting, SP-TOD effectively adapts to new functions in a zero-shot manner, \textit{by adding a few rules to current task schema}. In addition, SP-TOD surpasses the few-shot fine-tuning method augmented with machine teaching \cite{DBLP:conf/sigdial/WilliamsL17}, few-shot prompting strategy \cite{madotto2021few} by a significant margin.


% contribution (1) propose model to solve the problem; (2) functionality of the core part in the model; (3) conduct empirical experiments, results demonstrate ..

In summary, our contributions are four-fold.

\begin{itemize}\setlength{\itemsep}{0pt}

\item We propose SP-TOD, a schema-guided prompting method that allows readily building end-to-end task-oriented dialog systems on any new tasks in a zero-shot manner with only the task schema and little annotation required.

\item SP-TOD provides schema-compliant, knowledge-grounded, and human-like replies on any new tasks in a zero-shot way, by integrating database experience, domain-expert knowledge, and the robust language processing capabilities of LLMs.

\item SP-TOD has a strong potential for lifelong learning, as it can flexibly expand its skills to deal with new tasks by adding new schema rules with specialized functionalities.

\item Experimental results in zero-shot settings show that SP-TOD $(\RN{1})$ is on par with full-shot fine-tuning methods on Multiwoz, $(\RN{2})$ achieves superior performance compared to SOTA zero-shot transfer methods (fine-tuned on a large number of task-relevant data) on Multiwoz and comparable performance on STAR, $(\RN{3})$ significantly surpasses few-shot fine-tuning methods on RADDLE, $(\RN{4})$ considerably outperforms the few-shot fine-tuning method augmented with machine teaching, few-shot prompting strategy in the domain-extension setting.
\end{itemize}


% : $(\RN{1})$ the representation of the injected policy skeleton in the prompt resembles the format of the generation task, which is more instructive and interpret-able to the language models than independent descriptions; $(\RN{2})$ the frozen LLMs, pre-trained on a large volume of text data, have significant zero-shot skills to produce acceptable replies; $(\RN{3})$ our manually-designed policy skeleton contains more human-like template responses than the generated ones using the approach proposed in \citet{DBLP:conf/emnlp/KaleR20}. 


==> section/limitations.tex <==
%Data Contamination Data contamination (Brown et al., 2020) in prompt-based fewshot learning refers to the possible appearance of testing samples in the LM pre-training step. Verifying data contamination is challenging, especially when the LM training data are not released (e.g., GPT-2 (Radford et al., 2019)) and the dataset used for training the LM is extremely large (e.g., The Pile (Gao et al., 2020a)). Therefore, we cannot assume a lack of data contamination in our experiments, and a more thorough examination is left to future work.
%% manually-crafted task rules
\subsection{Manually-crafted schema rules.}
